Bar-Natan Homology for null homologous links in \mathbb{RP}^3

In this paper, we introduce Bar-Natan homology for null homologous links in \mathbb{RP}^3 over the field of two elements. It is a deformation of the Khovanov homology in \mathbb{RP}^3 defined by Asaeda, Przytycki and Sikora. We also define an s-invariant from this deformation using the same recipe as for links in S^3, and prove some genus bound using it. The key ingredient is the notion of twisted orientation for null homologous links and cobordisms in \mathbb{RP}^3.

==> biblio.tex <==
@article{bar2002khovanov,
	title={On Khovanov’s categorification of the Jones polynomial},
	author={Bar-Natan, Dror},
	journal={Algebraic \& Geometric Topology},
	volume={2},
	number={1},
	pages={337--370},
	year={2002},
	publisher={Mathematical Sciences Publishers}
}


@article{ozsvath2005heegaard,
	title={On the Heegaard Floer homology of branched double-covers},
	author={Ozsv{\'a}th, Peter and Szab{\'o}, Zolt{\'a}n},
	journal={Advances in Mathematics},
	volume={194},
	number={1},
	pages={1--33},
	year={2005},
	publisher={Elsevier}
}

@article{ozsvath2003absolutely,
	title={Absolutely graded Floer homologies and intersection forms for four-manifolds with boundary},
	author={Ozsv{\'a}th, Peter and Szab{\'o}, Zolt{\'a}n},
	journal={Advances in Mathematics},
	volume={173},
	number={2},
	pages={179--261},
	year={2003},
	publisher={Elsevier}
}

@article{drobotukhina1994classification,
	title={Classification of links in RP3 with at most six crossings},
	author={Drobotukhina, Yu V},
	journal={Advances in Soviet mathematics},
	volume={18},
	number={1},
	pages={87--121},
	year={1994}
}

@article{manolescu2010heegaard,
	title={Heegaard Floer homology and integer surgeries on links},
	author={Manolescu, Ciprian and Ozsv{\'a}th, Peter},
	journal={arXiv preprint arXiv:1011.1317},
	year={2010}
}


@article{ozsvath2004holomorphic,
	title={Holomorphic disks and three-manifold invariants: properties and applications},
	author={Ozsv{\'a}th, Peter and Szab{\'o}, Zolt{\'a}n},
	journal={Annals of Mathematics},
	pages={1159--1245},
	year={2004},
	publisher={JSTOR}
}

@article{roberts2013knot,
	title={On knot Floer homology in double branched covers},
	author={Roberts, Lawrence},
	journal={Geometry \& Topology},
	volume={17},
	number={1},
	pages={413--467},
	year={2013},
	publisher={Mathematical Sciences Publishers}
}

@article{asaeda2004categorification,
	title={Categorification of the Kauffman bracket skein module of I--bundles over surfaces},
	author={Asaeda, Marta M and Przytycki, J{\'o}zef H and Sikora, Adam S},
	journal={Algebraic \& Geometric Topology},
	volume={4},
	number={2},
	pages={1177--1210},
	year={2004},
	publisher={Mathematical Sciences Publishers}
}

@article{gabrovvsek2013categorification,
	title={THE CATEGORIFICATION OF THE KAUFFMAN BRACKET SKEIN MODULE OF},
	author={Gabrov{\v{s}}ek, Bo{\v{s}}tjan},
	journal={Bulletin of the Australian Mathematical Society},
	volume={88},
	number={3},
	pages={407--422},
	year={2013},
	publisher={Cambridge University Press}
}

@book{lickorish2012introduction,
	title={An introduction to knot theory},
	author={Lickorish, WB Raymond},
	volume={175},
	year={2012},
	publisher={Springer Science \& Business Media}
}

@article{hatcher2000algebraic,
	title={Algebraic topology},
	author={Hatcher, Allen},
	year={2000},
	publisher={Cambridge Univ. Press}
}

@article{hoste19932,
	title={The (2,$\infty$)-skein module of lens spaces: a generalization of the Jones polynomial},
	author={Hoste, Jim and Przytycki, J{\'o}zef H},
	journal={Journal of Knot Theory and Its Ramifications},
	volume={2},
	number={03},
	pages={321--333},
	year={1993},
	publisher={World Scientific}
}
